Towards Unbiased and Robust Spatio-Temporal Scene Graph Generation and Anticipation

Spatio-Temporal Scene Graphs (STSGs) provide a concise and expressive representation of dynamic scenes by modeling objects and their evolving relationships over time. However, real-world visual relationships often exhibit a long-tailed distribution, causing existing methods for tasks like Video Scene Graph Generation (VidSGG) and Scene Graph Anticipation (SGA) to produce biased scene graphs. To this end, we propose ImparTail, a novel training framework that leverages loss masking and curriculum learning to mitigate bias in the generation and anticipation of spatio-temporal scene graphs. Unlike prior methods that add extra architectural components to learn unbiased estimators, we propose an impartial training objective that reduces the dominance of head classes during learning and focuses on underrepresented tail relationships. Our curriculum-driven mask generation strategy further empowers the model to adaptively adjust its bias mitigation strategy over time, enabling more balanced and robust estimations. To thoroughly assess performance under various distribution shifts, we also introduce two new tasks Robust Spatio-Temporal Scene Graph Generation and Robust Scene Graph Anticipation offering a challenging benchmark for evaluating the resilience of STSG models. Extensive experiments on the Action Genome dataset demonstrate the superior unbiased performance and robustness of our method compared to existing baselines.

==> paper_sec/backup.tex <==
% This stands in contrast to techniques like curriculum by smoothing \cite{sinha_et_al_curr_by_smooth_2020} and curriculum dropout \cite{morerio_et_al_cr_drop_2017}, which focus on regularizing deep features without selective data sampling. 





% To address these issues, some researchers treat the selection of the next task as a stochastic policy that adapts to optimize learning progress \cite{graves_et_al_auto_cr_2017}. Other studies focus on leveraging prior knowledge about the difficulty of training examples to sample mini-batches non-uniformly \cite{hacohen_et_al_cl_tdn_2019}. 


% This added complexity could increase implementation difficulty and computational cost, potentially undermining training efficiency. Secondly, determining which examples should be prioritized during the early stages of learning is complex. The conventional "easy to hard" strategy is not universally effective; in some scenarios, emphasizing difficult-to-learn samples can be more beneficial, leading to what is known as a "hard to easy" anti-curriculum.

% Various indicators of learning progress, such as prediction gain and complexity gain, serve as reward signals to guide this process. Multi-armed bandit algorithms are employed to identify policies that maximize overall progress. This approach shares similarities with active learning, where such gain signals inform decisions about which data points to label next.


% Strategies include knowledge transfer from networks pre-trained on large datasets like ImageNet and bootstrapping through self-tutoring, where a network trained without a curriculum is used to rank training data for subsequent curriculum-based training.

==> paper_sec/tables/sga_mean_recall_sgcls_predcls.tex <==
\begin{table*}[!h]
    \centering
    \captionsetup{font=small}
    \caption{SGCLS and PREDCLS Mean Recall Results for SGA.}
    \label{tab:sgg_mean_recall_results}
    \renewcommand{\arraystretch}{1.2} 
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l|ccccccccc|ccccccccc}
    \hline
         \multirow{3}{*}{$\mathcal{F}$} & \multirow{3}{*}{Method} & \multicolumn{9}{c}{\textbf{SGCLS}} & \multicolumn{9}{c}{\textbf{PREDCLS}} \\ 
        \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
          & & \multicolumn{3}{c}{\textbf{With Constraint}} & \multicolumn{3}{c}{\textbf{No Constraint}} & \multicolumn{3}{c}{\textbf{Semi Constraint}} & \multicolumn{3}{c}{\textbf{With Constraint}} & \multicolumn{3}{c}{\textbf{No Constraint}} & \multicolumn{3}{c}{\textbf{Semi Constraint}} \\ 
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17} \cmidrule(lr){18-20} 
       &   & \textbf{@10} & \textbf{@20} & \textbf{@50} & \textbf{@10} & \textbf{@20} & \textbf{@50}  & \textbf{@10} & \textbf{@20} & \textbf{@50}  & \textbf{@10} & \textbf{@20} & \textbf{@50}  & \textbf{@10} & \textbf{@20} & \textbf{@50}  & \textbf{@10} & \textbf{@20} & \textbf{@50}  \\ \hline
        \multirow{12}{*}{0.3} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 10.6 & 11.5 & 11.5 & 15.7 & 25.7 & 47.4 & 4.8 & 4.8 & 4.8 & 13.9 & 16.2 & 16.3 & 19.2 & 31.2 & 57.4 & 6.9 & 7.0 & 7.0  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{12.1} & \cellcolor{highlightColor} \textbf{12.9} & \cellcolor{highlightColor} \textbf{12.9} & \cellcolor{highlightColor} \textbf{15.9} & \cellcolor{highlightColor} \textbf{26.0} & \cellcolor{highlightColor} \textbf{46.8} & \cellcolor{highlightColor} \textbf{2.9} & \cellcolor{highlightColor} \textbf{2.9} & \cellcolor{highlightColor} \textbf{2.9} & \cellcolor{highlightColor} \textbf{14.9} & \cellcolor{highlightColor} \textbf{16.9} & \cellcolor{highlightColor} \textbf{17.0} & \cellcolor{highlightColor} \textbf{20.6} & \cellcolor{highlightColor} \textbf{33.5} & \cellcolor{highlightColor} \textbf{57.5} & \cellcolor{highlightColor} \textbf{3.2} & \cellcolor{highlightColor} \textbf{3.2} & \cellcolor{highlightColor} \textbf{3.2}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 11.5 & 12.6 & 12.6 & 17.9 & 28.1 & 48.8 & 5.2 & 5.2 & 5.2 & 14.8 & 17.1 & 17.1 & 21.4 & 32.9 & 55.8 & 6.2 & 6.2 & 6.2  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{14.9} & \cellcolor{highlightColor} \textbf{15.8} & \cellcolor{highlightColor} \textbf{15.8} & \cellcolor{highlightColor} \textbf{20.6} & \cellcolor{highlightColor} \textbf{29.8} & \cellcolor{highlightColor} \textbf{49.8} & \cellcolor{highlightColor} \textbf{2.8} & \cellcolor{highlightColor} \textbf{2.8} & \cellcolor{highlightColor} \textbf{2.8} & \cellcolor{highlightColor} \textbf{18.6} & \cellcolor{highlightColor} \textbf{21.9} & \cellcolor{highlightColor} \textbf{21.9} & \cellcolor{highlightColor} \textbf{19.9} & \cellcolor{highlightColor} \textbf{34.2} & \cellcolor{highlightColor} \textbf{60.1} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{3.9}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 12.6 & 13.6 & 13.6 & 18.5 & 28.7 & 48.8 & 5.3 & 5.3 & 5.3 & 15.9 & 18.5 & 18.6 & 23.1 & 35.5 & 59.2 & 8.9 & 9.4 & 9.4  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{17.6} & \cellcolor{highlightColor} \textbf{18.9} & \cellcolor{highlightColor} \textbf{18.9} & \cellcolor{highlightColor} \textbf{21.2} & \cellcolor{highlightColor} \textbf{31.5} & \cellcolor{highlightColor} \textbf{49.2} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{17.8} & \cellcolor{highlightColor} \textbf{20.4} & \cellcolor{highlightColor} \textbf{20.4} & \cellcolor{highlightColor} \textbf{21.7} & \cellcolor{highlightColor} \textbf{35.7} & \cellcolor{highlightColor} \textbf{59.9} & \cellcolor{highlightColor} \textbf{3.7} & \cellcolor{highlightColor} \textbf{3.7} & \cellcolor{highlightColor} \textbf{3.7}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 13.0 & 14.0 & 14.0 & 17.9 & 28.6 & 49.2 & 4.2 & 4.3 & 4.3 & 15.1 & 17.5 & 17.5 & 21.2 & 34.3 & 57.4 & 6.2 & 6.3 & 6.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{16.4} & \cellcolor{highlightColor} \textbf{17.8} & \cellcolor{highlightColor} \textbf{17.8} & \cellcolor{highlightColor} \textbf{21.0} & \cellcolor{highlightColor} \textbf{31.6} & \cellcolor{highlightColor} \textbf{50.8} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{17.1} & \cellcolor{highlightColor} \textbf{19.7} & \cellcolor{highlightColor} \textbf{19.7} & \cellcolor{highlightColor} \textbf{20.1} & \cellcolor{highlightColor} \textbf{33.5} & \cellcolor{highlightColor} \textbf{58.4} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{3.9}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 9.4 & 10.5 & 10.5 & 14.3 & 23.3 & 44.6 & 2.7 & 2.8 & 2.8 & 15.2 & 17.9 & 18.0 & 22.2 & 34.5 & 56.7 & 9.7 & 11.2 & 11.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 13.5 & 15.2 & 15.2 & 20.6 & 31.2 & 49.8 & 6.4 & 6.5 & 6.5 & 16.1 & 19.2 & 19.3 & 23.1 & 35.7 & 57.7 & 8.8 & 9.2 & 9.2  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        \multirow{12}{*}{0.5} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 12.4 & 13.5 & 13.5 & 17.9 & 29.4 & 49.5 & 5.2 & 5.2 & 5.2 & 15.9 & 18.9 & 18.9 & 22.6 & 36.2 & 62.3 & 7.6 & 7.7 & 7.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{14.3} & \cellcolor{highlightColor} \textbf{15.2} & \cellcolor{highlightColor} \textbf{15.2} & \cellcolor{highlightColor} \textbf{18.3} & \cellcolor{highlightColor} \textbf{29.1} & \cellcolor{highlightColor} \textbf{48.2} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{16.3} & \cellcolor{highlightColor} \textbf{18.6} & \cellcolor{highlightColor} \textbf{18.6} & \cellcolor{highlightColor} \textbf{21.9} & \cellcolor{highlightColor} \textbf{35.8} & \cellcolor{highlightColor} \textbf{61.9} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 13.4 & 14.8 & 14.8 & 20.2 & 32.3 & 50.9 & 6.4 & 6.5 & 6.5 & 16.9 & 19.6 & 19.6 & 23.8 & 36.7 & 60.5 & 7.1 & 7.2 & 7.2  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{17.3} & \cellcolor{highlightColor} \textbf{18.6} & \cellcolor{highlightColor} \textbf{18.6} & \cellcolor{highlightColor} \textbf{22.6} & \cellcolor{highlightColor} \textbf{33.7} & \cellcolor{highlightColor} \textbf{50.7} & \cellcolor{highlightColor} \textbf{3.2} & \cellcolor{highlightColor} \textbf{3.2} & \cellcolor{highlightColor} \textbf{3.2} & \cellcolor{highlightColor} \textbf{20.8} & \cellcolor{highlightColor} \textbf{24.2} & \cellcolor{highlightColor} \textbf{24.3} & \cellcolor{highlightColor} \textbf{21.5} & \cellcolor{highlightColor} \textbf{36.6} & \cellcolor{highlightColor} \textbf{63.8} & \cellcolor{highlightColor} \textbf{4.4} & \cellcolor{highlightColor} \textbf{4.4} & \cellcolor{highlightColor} \textbf{4.4}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 14.3 & 15.8 & 15.8 & 20.9 & 32.5 & 50.1 & 5.6 & 5.6 & 5.6 & 17.8 & 20.9 & 21.0 & 25.2 & 39.4 & 63.5 & 9.2 & 9.6 & 9.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{20.2} & \cellcolor{highlightColor} \textbf{22.0} & \cellcolor{highlightColor} \textbf{22.0} & \cellcolor{highlightColor} \textbf{24.0} & \cellcolor{highlightColor} \textbf{34.9} & \cellcolor{highlightColor} \textbf{50.5} & \cellcolor{highlightColor} \textbf{4.1} & \cellcolor{highlightColor} \textbf{4.1} & \cellcolor{highlightColor} \textbf{4.1} & \cellcolor{highlightColor} \textbf{19.9} & \cellcolor{highlightColor} \textbf{22.7} & \cellcolor{highlightColor} \textbf{22.8} & \cellcolor{highlightColor} \textbf{23.7} & \cellcolor{highlightColor} \textbf{39.2} & \cellcolor{highlightColor} \textbf{64.1} & \cellcolor{highlightColor} \textbf{4.3} & \cellcolor{highlightColor} \textbf{4.3} & \cellcolor{highlightColor} \textbf{4.3}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 15.0 & 16.3 & 16.3 & 19.9 & 32.3 & 50.6 & 4.5 & 4.5 & 4.5 & 17.1 & 20.0 & 20.0 & 23.2 & 37.3 & 62.9 & 6.0 & 6.1 & 6.1  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{18.6} & \cellcolor{highlightColor} \textbf{20.1} & \cellcolor{highlightColor} \textbf{20.1} & \cellcolor{highlightColor} \textbf{22.6} & \cellcolor{highlightColor} \textbf{35.2} & \cellcolor{highlightColor} \textbf{52.5} & \cellcolor{highlightColor} \textbf{3.7} & \cellcolor{highlightColor} \textbf{3.7} & \cellcolor{highlightColor} \textbf{3.7} & \cellcolor{highlightColor} \textbf{21.1} & \cellcolor{highlightColor} \textbf{24.5} & \cellcolor{highlightColor} \textbf{24.5} & \cellcolor{highlightColor} \textbf{23.3} & \cellcolor{highlightColor} \textbf{38.4} & \cellcolor{highlightColor} \textbf{63.2} & \cellcolor{highlightColor} \textbf{4.5} & \cellcolor{highlightColor} \textbf{4.5} & \cellcolor{highlightColor} \textbf{4.5}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 11.2 & 12.8 & 12.8 & 16.9 & 26.3 & 45.7 & 3.2 & 3.2 & 3.2 & 17.5 & 20.7 & 20.9 & 24.9 & 38.0 & 61.8 & 9.7 & 10.6 & 10.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 15.2 & 17.5 & 17.5 & 22.9 & 34.3 & 51.0 & 7.0 & 7.1 & 7.1 & 18.2 & 21.7 & 21.8 & 25.0 & 39.0 & 62.7 & 9.3 & 9.7 & 9.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        \multirow{12}{*}{0.7} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 15.6 & 16.8 & 16.8 & 23.5 & 36.4 & 55.4 & 6.3 & 6.4 & 6.4 & 18.8 & 21.6 & 21.6 & 27.6 & 43.6 & 73.2 & 8.6 & 8.7 & 8.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{17.1} & \cellcolor{highlightColor} \textbf{18.1} & \cellcolor{highlightColor} \textbf{18.1} & \cellcolor{highlightColor} \textbf{22.8} & \cellcolor{highlightColor} \textbf{35.1} & \cellcolor{highlightColor} \textbf{54.7} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{19.7} & \cellcolor{highlightColor} \textbf{22.0} & \cellcolor{highlightColor} \textbf{22.0} & \cellcolor{highlightColor} \textbf{26.9} & \cellcolor{highlightColor} \textbf{43.8} & \cellcolor{highlightColor} \textbf{73.2} & \cellcolor{highlightColor} \textbf{4.0} & \cellcolor{highlightColor} \textbf{4.0} & \cellcolor{highlightColor} \textbf{4.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 15.3 & 16.6 & 16.6 & 24.2 & 38.0 & 56.7 & 7.4 & 7.4 & 7.4 & 20.2 & 22.8 & 22.8 & 29.0 & 44.7 & 71.6 & 8.2 & 8.3 & 8.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{20.7} & \cellcolor{highlightColor} \textbf{22.1} & \cellcolor{highlightColor} \textbf{22.1} & \cellcolor{highlightColor} \textbf{27.7} & \cellcolor{highlightColor} \textbf{40.8} & \cellcolor{highlightColor} \textbf{57.9} & \cellcolor{highlightColor} \textbf{3.8} & \cellcolor{highlightColor} \textbf{3.8} & \cellcolor{highlightColor} \textbf{3.8} & \cellcolor{highlightColor} \textbf{25.2} & \cellcolor{highlightColor} \textbf{28.8} & \cellcolor{highlightColor} \textbf{28.8} & \cellcolor{highlightColor} \textbf{27.0} & \cellcolor{highlightColor} \textbf{44.6} & \cellcolor{highlightColor} \textbf{75.0} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{5.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 17.2 & 18.6 & 18.6 & 25.3 & 38.3 & 56.1 & 6.2 & 6.3 & 6.3 & 21.9 & 25.0 & 25.0 & 31.2 & 47.0 & 75.4 & 10.6 & 11.0 & 11.0  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{25.6} & \cellcolor{highlightColor} \textbf{27.4} & \cellcolor{highlightColor} \textbf{27.4} & \cellcolor{highlightColor} \textbf{29.8} & \cellcolor{highlightColor} \textbf{43.9} & \cellcolor{highlightColor} \textbf{57.6} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{25.8} & \cellcolor{highlightColor} \textbf{29.1} & \cellcolor{highlightColor} \textbf{29.1} & \cellcolor{highlightColor} \textbf{31.1} & \cellcolor{highlightColor} \textbf{49.2} & \cellcolor{highlightColor} \textbf{76.5} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{5.0} & \cellcolor{highlightColor} \textbf{5.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 18.1 & 19.4 & 19.4 & 24.8 & 39.5 & 57.3 & 5.4 & 5.4 & 5.4 & 20.8 & 23.8 & 23.8 & 28.6 & 46.1 & 73.8 & 6.9 & 7.0 & 7.0  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{23.6} & \cellcolor{highlightColor} \textbf{25.5} & \cellcolor{highlightColor} \textbf{25.5} & \cellcolor{highlightColor} \textbf{28.1} & \cellcolor{highlightColor} \textbf{42.2} & \cellcolor{highlightColor} \textbf{58.5} & \cellcolor{highlightColor} \textbf{4.3} & \cellcolor{highlightColor} \textbf{4.3} & \cellcolor{highlightColor} \textbf{4.3} & \cellcolor{highlightColor} \textbf{28.3} & \cellcolor{highlightColor} \textbf{32.5} & \cellcolor{highlightColor} \textbf{32.5} & \cellcolor{highlightColor} \textbf{31.4} & \cellcolor{highlightColor} \textbf{49.7} & \cellcolor{highlightColor} \textbf{75.7} & \cellcolor{highlightColor} \textbf{5.5} & \cellcolor{highlightColor} \textbf{5.5} & \cellcolor{highlightColor} \textbf{5.5}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 13.6 & 15.1 & 15.1 & 20.5 & 32.4 & 52.8 & 3.7 & 3.7 & 3.7 & 20.7 & 24.0 & 24.0 & 29.8 & 45.2 & 72.0 & 10.1 & 10.6 & 10.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 17.9 & 19.9 & 19.9 & 27.0 & 40.2 & 57.2 & 8.0 & 8.1 & 8.1 & 21.0 & 24.6 & 24.6 & 30.2 & 45.4 & 72.8 & 10.5 & 10.7 & 10.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        \multirow{12}{*}{0.9} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 18.4 & 19.6 & 19.6 & 30.0 & 44.0 & 60.0 & 7.7 & 7.8 & 7.8 & 22.9 & 25.0 & 25.0 & 36.1 & 54.9 & 81.8 & 9.9 & 10.1 & 10.1  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{21.5} & \cellcolor{highlightColor} \textbf{22.4} & \cellcolor{highlightColor} \textbf{22.4} & \cellcolor{highlightColor} \textbf{29.8} & \cellcolor{highlightColor} \textbf{43.8} & \cellcolor{highlightColor} \textbf{61.5} & \cellcolor{highlightColor} \textbf{5.2} & \cellcolor{highlightColor} \textbf{5.2} & \cellcolor{highlightColor} \textbf{5.2} & \cellcolor{highlightColor} \textbf{25.2} & \cellcolor{highlightColor} \textbf{27.2} & \cellcolor{highlightColor} \textbf{27.2} & \cellcolor{highlightColor} \textbf{35.9} & \cellcolor{highlightColor} \textbf{55.4} & \cellcolor{highlightColor} \textbf{83.2} & \cellcolor{highlightColor} \textbf{4.6} & \cellcolor{highlightColor} \textbf{4.6} & \cellcolor{highlightColor} \textbf{4.6}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 18.3 & 19.4 & 19.4 & 30.9 & 45.4 & 63.3 & 8.4 & 8.5 & 8.5 & 24.0 & 26.0 & 26.0 & 36.8 & 54.7 & 80.3 & 9.6 & 9.6 & 9.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{24.4} & \cellcolor{highlightColor} \textbf{25.8} & \cellcolor{highlightColor} \textbf{25.8} & \cellcolor{highlightColor} \textbf{35.0} & \cellcolor{highlightColor} \textbf{47.8} & \cellcolor{highlightColor} \textbf{65.0} & \cellcolor{highlightColor} \textbf{4.6} & \cellcolor{highlightColor} \textbf{4.6} & \cellcolor{highlightColor} \textbf{4.6} & \cellcolor{highlightColor} \textbf{31.8} & \cellcolor{highlightColor} \textbf{35.0} & \cellcolor{highlightColor} \textbf{35.0} & \cellcolor{highlightColor} \textbf{37.3} & \cellcolor{highlightColor} \textbf{56.1} & \cellcolor{highlightColor} \textbf{90.7} & \cellcolor{highlightColor} \textbf{5.7} & \cellcolor{highlightColor} \textbf{5.7} & \cellcolor{highlightColor} \textbf{5.7}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 21.2 & 22.5 & 22.5 & 32.4 & 46.9 & 60.6 & 7.8 & 7.9 & 7.9 & 28.8 & 31.3 & 31.3 & 42.5 & 60.8 & 84.8 & 14.2 & 14.7 & 14.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{32.6} & \cellcolor{highlightColor} \textbf{34.2} & \cellcolor{highlightColor} \textbf{34.2} & \cellcolor{highlightColor} \textbf{40.9} & \cellcolor{highlightColor} \textbf{52.1} & \cellcolor{highlightColor} \textbf{63.8} & \cellcolor{highlightColor} \textbf{7.5} & \cellcolor{highlightColor} \textbf{7.5} & \cellcolor{highlightColor} \textbf{7.5} & \cellcolor{highlightColor} \textbf{36.7} & \cellcolor{highlightColor} \textbf{40.3} & \cellcolor{highlightColor} \textbf{40.3} & \cellcolor{highlightColor} \textbf{46.3} & \cellcolor{highlightColor} \textbf{64.4} & \cellcolor{highlightColor} \textbf{91.4} & \cellcolor{highlightColor} \textbf{7.0} & \cellcolor{highlightColor} \textbf{7.0} & \cellcolor{highlightColor} \textbf{7.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 22.2 & 23.4 & 23.4 & 33.0 & 49.0 & 64.2 & 7.5 & 7.5 & 7.5 & 27.0 & 29.4 & 29.4 & 39.0 & 58.8 & 83.2 & 8.8 & 9.0 & 9.0  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{30.9} & \cellcolor{highlightColor} \textbf{32.2} & \cellcolor{highlightColor} \textbf{32.2} & \cellcolor{highlightColor} \textbf{38.3} & \cellcolor{highlightColor} \textbf{52.6} & \cellcolor{highlightColor} \textbf{67.3} & \cellcolor{highlightColor} \textbf{6.1} & \cellcolor{highlightColor} \textbf{6.1} & \cellcolor{highlightColor} \textbf{6.1} & \cellcolor{highlightColor} \textbf{38.7} & \cellcolor{highlightColor} \textbf{42.8} & \cellcolor{highlightColor} \textbf{42.8} & \cellcolor{highlightColor} \textbf{46.9} & \cellcolor{highlightColor} \textbf{65.7} & \cellcolor{highlightColor} \textbf{91.0} & \cellcolor{highlightColor} \textbf{7.0} & \cellcolor{highlightColor} \textbf{7.0} & \cellcolor{highlightColor} \textbf{7.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 16.6 & 17.9 & 17.9 & 27.4 & 41.7 & 61.1 & 4.4 & 4.4 & 4.4 & 25.1 & 27.6 & 27.6 & 37.2 & 54.3 & 81.5 & 10.5 & 10.6 & 10.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 21.0 & 22.6 & 22.6 & 33.2 & 48.2 & 64.3 & 8.9 & 9.1 & 9.1 & 24.7 & 27.3 & 27.3 & 37.3 & 54.0 & 80.5 & 11.3 & 11.5 & 11.5  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} \cmidrule(lr){12-20} 
    \end{tabular}
    }
\end{table*}


==> paper_sec/tables/sga_mean_recall_sgdet.tex <==
\begin{table}[!h]
    \centering
    \captionsetup{font=small}
    \caption{SGDET Mean Recall Results for SGA.}
    \label{tab:sgg_mean_recall_results}
    \renewcommand{\arraystretch}{1.2} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|ccccccccc}
    \hline
        \multirow{3}{*}{$\mathcal{F}$} & \multirow{3}{*}{Method} & \multicolumn{9}{c}{\textbf{SGDET}} \\ 
        \cmidrule(lr){3-11} 
         & & \multicolumn{3}{c}{\textbf{With Constraint}} & \multicolumn{3}{c}{\textbf{No Constraint}} & \multicolumn{3}{c}{\textbf{Semi Constraint}} \\ 
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}  
     &    & \textbf{@10} & \textbf{@20} & \textbf{@50} & \textbf{@10} & \textbf{@20} & \textbf{@50}  & \textbf{@10} & \textbf{@20} & \textbf{@50}  \\ \hline
        \multirow{12}{*}{0.3} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 6.1 & 12.2 & 13.5 & 11.9 & 17.4 & 33.5 & 5.7 & 7.9 & 8.0  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{8.3} & \cellcolor{highlightColor} \textbf{15.3} & \cellcolor{highlightColor} \textbf{16.6} & \cellcolor{highlightColor} \textbf{11.2} & \cellcolor{highlightColor} \textbf{18.2} & \cellcolor{highlightColor} \textbf{33.8} & \cellcolor{highlightColor} \textbf{3.1} & \cellcolor{highlightColor} \textbf{3.1} & \cellcolor{highlightColor} \textbf{3.1}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 6.9 & 13.1 & 14.3 & 12.7 & 19.1 & 35.2 & 5.2 & 6.1 & 6.1  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{6.8} & \cellcolor{highlightColor} \textbf{11.8} & \cellcolor{highlightColor} \textbf{12.5} & \cellcolor{highlightColor} \textbf{7.8} & \cellcolor{highlightColor} \textbf{14.6} & \cellcolor{highlightColor} \textbf{29.7} & \cellcolor{highlightColor} \textbf{2.7} & \cellcolor{highlightColor} \textbf{2.7} & \cellcolor{highlightColor} \textbf{2.7}  \\ 
          \cmidrule(lr){3-11} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 7.6 & 15.3 & 16.9 & 13.1 & 20.2 & 36.2 & 5.0 & 6.4 & 6.4  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{8.9} & \cellcolor{highlightColor} \textbf{17.9} & \cellcolor{highlightColor} \textbf{19.7} & \cellcolor{highlightColor} \textbf{11.1} & \cellcolor{highlightColor} \textbf{18.5} & \cellcolor{highlightColor} \textbf{36.5} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{3.6}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 7.1 & 12.8 & 13.8 & 11.5 & 17.8 & 34.1 & 4.9 & 5.7 & 5.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{9.3} & \cellcolor{highlightColor} \textbf{18.4} & \cellcolor{highlightColor} \textbf{20.2} & \cellcolor{highlightColor} \textbf{12.8} & \cellcolor{highlightColor} \textbf{21.8} & \cellcolor{highlightColor} \textbf{37.5} & \cellcolor{highlightColor} \textbf{3.1} & \cellcolor{highlightColor} \textbf{3.1} & \cellcolor{highlightColor} \textbf{3.1}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 5.5 & 11.9 & 19.0 & 12.6 & 19.3 & 32.7 & 4.7 & 7.9 & 9.9  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 5.9 & 13.4 & 17.2 & 14.3 & 22.0 & 36.4 & 4.3 & 6.1 & 6.4  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        \multirow{12}{*}{0.5} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 6.5 & 13.2 & 14.7 & 12.6 & 18.3 & 36.1 & 6.0 & 8.3 & 8.4  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{8.9} & \cellcolor{highlightColor} \textbf{16.3} & \cellcolor{highlightColor} \textbf{18.0} & \cellcolor{highlightColor} \textbf{11.8} & \cellcolor{highlightColor} \textbf{19.5} & \cellcolor{highlightColor} \textbf{35.8} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{3.3}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 7.2 & 14.0 & 15.4 & 13.7 & 20.5 & 38.1 & 5.5 & 6.6 & 6.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{7.2} & \cellcolor{highlightColor} \textbf{12.7} & \cellcolor{highlightColor} \textbf{13.4} & \cellcolor{highlightColor} \textbf{8.2} & \cellcolor{highlightColor} \textbf{15.6} & \cellcolor{highlightColor} \textbf{32.9} & \cellcolor{highlightColor} \textbf{2.9} & \cellcolor{highlightColor} \textbf{2.9} & \cellcolor{highlightColor} \textbf{2.9}  \\ 
          \cmidrule(lr){3-11} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 7.9 & 16.4 & 18.4 & 13.9 & 21.3 & 38.5 & 5.1 & 6.6 & 6.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{9.3} & \cellcolor{highlightColor} \textbf{18.7} & \cellcolor{highlightColor} \textbf{20.9} & \cellcolor{highlightColor} \textbf{12.1} & \cellcolor{highlightColor} \textbf{20.0} & \cellcolor{highlightColor} \textbf{39.6} & \cellcolor{highlightColor} \textbf{3.9} & \cellcolor{highlightColor} \textbf{4.0} & \cellcolor{highlightColor} \textbf{4.0}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 7.4 & 13.4 & 14.6 & 11.8 & 18.2 & 36.1 & 5.0 & 5.7 & 5.7  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{9.8} & \cellcolor{highlightColor} \textbf{19.8} & \cellcolor{highlightColor} \textbf{21.9} & \cellcolor{highlightColor} \textbf{13.5} & \cellcolor{highlightColor} \textbf{22.9} & \cellcolor{highlightColor} \textbf{40.7} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{3.3} & \cellcolor{highlightColor} \textbf{3.3}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 5.8 & 12.6 & 16.9 & 14.0 & 22.3 & 36.5 & 4.7 & 7.8 & 9.9  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 6.4 & 13.7 & 18.3 & 15.4 & 23.7 & 38.7 & 4.6 & 6.9 & 7.2  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        \multirow{12}{*}{0.7} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 7.4 & 14.7 & 16.4 & 13.8 & 20.4 & 39.7 & 6.7 & 9.3 & 9.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{10.0} & \cellcolor{highlightColor} \textbf{18.3} & \cellcolor{highlightColor} \textbf{20.0} & \cellcolor{highlightColor} \textbf{13.4} & \cellcolor{highlightColor} \textbf{21.6} & \cellcolor{highlightColor} \textbf{39.6} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{3.6} & \cellcolor{highlightColor} \textbf{3.6}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 8.3 & 15.8 & 17.1 & 15.1 & 22.9 & 41.0 & 6.1 & 7.3 & 7.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{8.1} & \cellcolor{highlightColor} \textbf{13.7} & \cellcolor{highlightColor} \textbf{14.7} & \cellcolor{highlightColor} \textbf{9.3} & \cellcolor{highlightColor} \textbf{17.3} & \cellcolor{highlightColor} \textbf{35.7} & \cellcolor{highlightColor} \textbf{3.0} & \cellcolor{highlightColor} \textbf{3.0} & \cellcolor{highlightColor} \textbf{3.0}  \\ 
          \cmidrule(lr){3-11} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 9.1 & 18.2 & 20.2 & 15.7 & 23.7 & 41.9 & 5.8 & 7.3 & 7.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{10.9} & \cellcolor{highlightColor} \textbf{21.9} & \cellcolor{highlightColor} \textbf{24.1} & \cellcolor{highlightColor} \textbf{14.0} & \cellcolor{highlightColor} \textbf{23.2} & \cellcolor{highlightColor} \textbf{43.7} & \cellcolor{highlightColor} \textbf{4.3} & \cellcolor{highlightColor} \textbf{4.4} & \cellcolor{highlightColor} \textbf{4.4}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 8.4 & 14.8 & 16.0 & 13.2 & 20.0 & 38.8 & 5.6 & 6.3 & 6.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{11.5} & \cellcolor{highlightColor} \textbf{23.1} & \cellcolor{highlightColor} \textbf{25.2} & \cellcolor{highlightColor} \textbf{15.9} & \cellcolor{highlightColor} \textbf{26.7} & \cellcolor{highlightColor} \textbf{45.3} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 6.7 & 14.0 & 18.5 & 16.4 & 24.9 & 40.5 & 5.1 & 7.4 & 8.5  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 7.1 & 14.6 & 19.3 & 17.3 & 26.1 & 42.5 & 5.2 & 7.3 & 7.5  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        \multirow{12}{*}{0.9} &        STTran+~\cite{peddi_et_al_scene_sayer_2024} & 8.1 & 16.7 & 18.7 & 15.1 & 23.5 & 42.9 & 7.0 & 10.2 & 10.3  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{11.5} & \cellcolor{highlightColor} \textbf{22.1} & \cellcolor{highlightColor} \textbf{24.5} & \cellcolor{highlightColor} \textbf{16.6} & \cellcolor{highlightColor} \textbf{25.5} & \cellcolor{highlightColor} \textbf{44.7} & \cellcolor{highlightColor} \textbf{4.1} & \cellcolor{highlightColor} \textbf{4.1} & \cellcolor{highlightColor} \textbf{4.1}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr+~\cite{peddi_et_al_scene_sayer_2024} & 9.1 & 18.1 & 19.6 & 17.4 & 26.2 & 45.2 & 6.5 & 8.0 & 8.0  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{9.7} & \cellcolor{highlightColor} \textbf{16.9} & \cellcolor{highlightColor} \textbf{18.0} & \cellcolor{highlightColor} \textbf{11.3} & \cellcolor{highlightColor} \textbf{20.7} & \cellcolor{highlightColor} \textbf{40.9} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5} & \cellcolor{highlightColor} \textbf{3.5}  \\ 
          \cmidrule(lr){3-11} 
        &        STTran++~\cite{peddi_et_al_scene_sayer_2024} & 9.8 & 20.9 & 23.5 & 18.2 & 27.5 & 47.2 & 7.1 & 9.4 & 9.4  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{12.6} & \cellcolor{highlightColor} \textbf{27.1} & \cellcolor{highlightColor} \textbf{29.9} & \cellcolor{highlightColor} \textbf{18.8} & \cellcolor{highlightColor} \textbf{30.4} & \cellcolor{highlightColor} \textbf{51.4} & \cellcolor{highlightColor} \textbf{5.4} & \cellcolor{highlightColor} \textbf{5.5} & \cellcolor{highlightColor} \textbf{5.5}  \\ 
          \cmidrule(lr){3-11} 
        &        DSGDetr++~\cite{peddi_et_al_scene_sayer_2024} & 9.5 & 17.7 & 19.2 & 15.5 & 23.8 & 44.9 & 6.9 & 8.1 & 8.1  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{13.6} & \cellcolor{highlightColor} \textbf{27.8} & \cellcolor{highlightColor} \textbf{30.2} & \cellcolor{highlightColor} \textbf{21.2} & \cellcolor{highlightColor} \textbf{32.1} & \cellcolor{highlightColor} \textbf{51.2} & \cellcolor{highlightColor} \textbf{4.4} & \cellcolor{highlightColor} \textbf{4.4} & \cellcolor{highlightColor} \textbf{4.4}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerODE~\cite{peddi_et_al_scene_sayer_2024} & 7.0 & 15.6 & 21.0 & 18.9 & 28.6 & 45.2 & 5.1 & 6.9 & 7.2  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
        &        SceneSayerSDE~\cite{peddi_et_al_scene_sayer_2024} & 7.4 & 16.0 & 21.1 & 19.1 & 29.0 & 45.6 & 5.8 & 8.2 & 8.6  \\ 
        &        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0} & \cellcolor{highlightColor} \textbf{0.0}  \\ 
          \cmidrule(lr){3-11} 
    \end{tabular}
    }
\end{table}


==> paper_sec/tables/sgg_mean_recall_sgdet.tex <==
\begin{table}[!h]
    \centering
    \captionsetup{font=small}
    \caption{SGDET Mean Recall Results for VidSGG.}
    \label{tab:sgg_mean_recall_results}
    \renewcommand{\arraystretch}{1.2} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccccccc}
    \hline
         \multirow{3}{*}{Method} & \multicolumn{9}{c}{\textbf{SGDET}} \\ 
        \cmidrule(lr){2-10} 
          & \multicolumn{3}{c}{\textbf{With Constraint}} & \multicolumn{3}{c}{\textbf{No Constraint}} & \multicolumn{3}{c}{\textbf{Semi Constraint}} \\ 
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  
          & \textbf{@10} & \textbf{@20} & \textbf{@50} & \textbf{@10} & \textbf{@20} & \textbf{@50}  & \textbf{@10} & \textbf{@20} & \textbf{@50}  \\ \hline
        STTran~\cite{cong_et_al_sttran_2021} & 8.0 & 16.6 & 19.3 & 19.3 & 26.9 & 35.6 & 7.7 & 18.2 & 30.4  \\ 
        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{9.4} & \cellcolor{highlightColor} \textbf{21.5} & \cellcolor{highlightColor} \textbf{25.9} & \cellcolor{highlightColor} \textbf{23.5} & \cellcolor{highlightColor} \textbf{33.6} & \cellcolor{highlightColor} \textbf{43.8} & \cellcolor{highlightColor} \textbf{8.6} & \cellcolor{highlightColor} \textbf{21.8} & \cellcolor{highlightColor} \textbf{38.3}  \\ 
          \hline 
        DSGDetr~\cite{Feng_2021} & 6.7 & 14.7 & 19.1 & 23.3 & 29.8 & 36.0 & 6.5 & 16.0 & 30.4  \\ 
        \quad+\textbf{ImparTail(Ours)} & \cellcolor{highlightColor} \textbf{7.5} & \cellcolor{highlightColor} \textbf{17.8} & \cellcolor{highlightColor} \textbf{23.7} & \cellcolor{highlightColor} \textbf{27.5} & \cellcolor{highlightColor} \textbf{35.2} & \cellcolor{highlightColor} \textbf{43.3} & \cellcolor{highlightColor} \textbf{7.3} & \cellcolor{highlightColor} \textbf{18.4} & \cellcolor{highlightColor} \textbf{36.6}  \\ 
          \hline 
    \end{tabular}
    }
\end{table}


